Reason2Drive: Towards Interpretable and Chain-based Reasoning for Autonomous Driving

Large vision-language models (VLMs) have garnered increasing interest in autonomous driving areas, due to their advanced capabilities in complex reasoning tasks essential for highly autonomous vehicle behavior. Despite their potential, research in autonomous systems is hindered by the lack of datasets with annotated reasoning chains that explain the decision-making processes in driving. To bridge this gap, we present Reason2Drive, a benchmark dataset with over 600K video-text pairs, aimed at facilitating the study of interpretable reasoning in complex driving environments. We distinctly characterize the autonomous driving process as a sequential combination of perception, prediction, and reasoning steps, and the question-answer pairs are automatically collected from a diverse range of open-source outdoor driving datasets, including nuScenes, Waymo and ONCE. Moreover, we introduce a novel aggregated evaluation metric to assess chain-based reasoning performance in autonomous systems, addressing the semantic ambiguities of existing metrics such as BLEU and CIDEr. Based on the proposed benchmark, we conduct experiments to assess various existing VLMs, revealing insights into their reasoning capabilities. Additionally, we develop an efficient approach to empower VLMs to leverage object-level perceptual elements in both feature extraction and prediction, further enhancing their reasoning accuracy. The code and dataset will be released.

==> tables/gpt+downstream.tex <==
\begin{minipage}{\textwidth}
 \begin{minipage}[t]{0.5\textwidth}
  \centering
  \makeatletter\def\@captype{table}\makeatother\caption{Ablations on visual input and perception priors.}
  \resizebox{0.95\textwidth}{!}{
   \begin{tabular}{c|c|cc|cc}
   \midrule[1.0pt]
   Methods & LLM & Strict Reason & Reason & GPT-3.5 & GPT-4 \\
   \midrule[1.0pt]
   Blip-2 & OPT-2.7B & 0.332 & 0.450 & 0.479 & 0.458 \\
   InstructBLIP & FlanT5-XL & 0.377 & 0.489 & 0.532 & 0.501 \\
   MiniGPT-4 & Vicuna-7B & 0.352 & 0.469 & 0.519 & 0.467 \\
   \midrule
   Ours & Vicuna-7B & \textbf{0.561} & \textbf{0.593} & \textbf{0.643} & \textbf{0.628} \\
   \midrule[1.0pt]
   \end{tabular}}
 \end{minipage}
 \begin{minipage}[t]{0.45\textwidth}
  \centering
  \makeatletter\def\@captype{table}\makeatother\caption{Ablations on different settings of instructed vision decoder.}
  \resizebox{0.95\textwidth}{!}{
   \begin{tabular}{c|c|cccc}
   \midrule[1.0pt]
   \rowcolor[gray]{0.8}& & & & \multicolumn{2}{c}{RMSE} \\
   \rowcolor[gray]{0.8}\multirow{-2}{*}{Method} & \multirow{-2}{*}{LLM} & \multirow{-2}{*}{B $\uparrow$} & \multirow{-2}{*}{M $\uparrow$} & Speed $\downarrow$ & Steer $\downarrow$ \\
   \midrule[1.0pt]
   \multicolumn{5}{l}{\textit{Directly fine-tuned with control signals:}} \\
   \midrule[1.0pt]
   InstructBLIP & Vicuna-7B & 0.166 & 0.201 & 3.743 & 5.926 \\
   \midrule[1.0pt]
   \multicolumn{5}{l}{\textit{Additionally pre-trained on Reason2Drive:}} \\
   \midrule[1.0pt]
   InstructBLIP & Vicuna-7B & 0.192 & 0.237 & 3.086 & 5.151 \\
   Ours & Vicuna-7B & \textbf{0.213} & \textbf{0.269} & \textbf{2.842} & \textbf{4.866} \\
   \midrule[1.0pt]
   \end{tabular}}
 \end{minipage}
\end{minipage}

==> tables/more_downstream.tex <==
\begin{table}[thbp]
\renewcommand\arraystretch{1.5}
\setlength{\tabcolsep}{20pt}
\begin{center}
\vspace{-4mm}
\resizebox{1.0\linewidth}{0.04\textheight}{
\begin{tabular}{c|c|cccc}
\midrule[1.0pt]
\rowcolor[gray]{0.8}& & & & \multicolumn{2}{c}{RMSE} \\
\rowcolor[gray]{0.8}\multirow{-2}{*}{Method} & \multirow{-2}{*}{LLM} & \multirow{-2}{*}{B $\uparrow$} & \multirow{-2}{*}{M $\uparrow$} & Speed $\downarrow$ & Steer $\downarrow$ \\
\midrule[1.0pt]
LLaVA-1.5 & Vicuna-7B & 0.180 & 0.249 & 2.973 & 5.084 \\
LLaMA-VID & Vicuna-7B & 0.197 & 0.264 & 3.252 & 5.107 \\
Ours & Vicuna-7B & \textbf{0.213} & \textbf{0.269} & \textbf{2.842} & \textbf{4.866} \\
\midrule[1.0pt]
\end{tabular}}
\end{center}
\vspace{-7mm}
\caption{Evaluation of end-to-end tasks. B: B@4. M: METHOR.}
\label{tab-more_control}
\vspace{-4mm}
\end{table}

==> tables/more_visual.tex <==
\begin{table}[thbp]
\renewcommand\arraystretch{1.5}
\setlength{\tabcolsep}{20pt}
\begin{center}
\vspace{-4mm}
\resizebox{1.0\linewidth}{0.03\textheight}{
\begin{tabular}{c|c|ccc}
\midrule[1.0pt]
\rowcolor[gray]{0.8}Predictions & Metric & GLIP & FIBER & Ours \\
\midrule[1.0pt]
Bounding box & Accuracy $\uparrow$ & 0.698 & 0.763 & \textbf{0.806} \\
% \hline
\midrule[1.0pt]
\end{tabular}}
\end{center}
\vspace{-7mm}
\caption{The quality of predicted visual elements.}
\label{tab-more_bbox}
\vspace{-10mm}
\end{table}

==> tables/test_results.tex <==
\begin{table}[thbp]
\renewcommand\arraystretch{1.5}
\setlength{\tabcolsep}{20pt}
\begin{center}
\vspace{-3mm}
\resizebox{1.0\linewidth}{0.04\textheight}{
\begin{tabular}{c|c|cc|cccc}
\midrule[1.0pt]
\rowcolor[gray]{0.8}& & \multicolumn{2}{c|}{Reasoning metric} & \multicolumn{4}{c}{Captioning metric} \\
\rowcolor[gray]{0.8}\multirow{-2}{*}{Methods} & \multirow{-2}{*}{LLM} & ADRScore & ADRScore-S & B@4 & METEOR & ROUGE & CIDEr \\
% \midrule
\midrule[1.0pt]
InstructBLIP & Vicuna-7B & 0.342 & 0.183 & 0.362 & 0.319 & 0.453 & 0.251 \\
MiniGPT-4 & Vicuna-7B & 0.335 & 0.191 & 0.379 & 0.315 & 0.458 & 0.242 \\
\midrule
Ours & Vicuna-7B & \textbf{0.452} & \textbf{0.418} & \textbf{0.421} & \textbf{0.382} & \textbf{0.493} & \textbf{0.317} \\
\midrule[1.0pt]
\end{tabular}}
\end{center}
\vspace{-7mm}
\caption{Evaluation on newly appended test set.}
\label{tab-test}
\vspace{-6mm}
\end{table}
